Estimating and Improving Fairness with Adversarial Learning

Fairness and accountability are two essential pillars for trustworthy Artificial Intelligence (AI) in healthcare. However, the existing AI model may be biased in its decision marking. To tackle this issue, we propose an adversarial multi-task training strategy to simultaneously mitigate and detect bias in the deep learning-based medical image analysis system. Specifically, we propose to add a discrimination module against bias and a critical module that predicts unfairness within the base classification model. We further impose an orthogonality regularization to force the two modules to be independent during training. Hence, we can keep these deep learning tasks distinct from one another, and avoid collapsing them into a singular point on the manifold. Through this adversarial training method, the data from the underprivileged group, which is vulnerable to bias because of attributes such as sex and skin tone, are transferred into a domain that is neutral relative to these attributes. Furthermore, the critical module can predict fairness scores for the data with unknown sensitive attributes. We evaluate our framework on a large-scale public-available skin lesion dataset under various fairness evaluation metrics. The experiments demonstrate the effectiveness of our proposed method for estimating and improving fairness in the deep learning-based medical image analysis system.

==> 2-preliminaries.tex <==
\section{Related Works}

%Artificial Intelligence is now playing a more critical role in medical imaging analysis that involves high-stake decision, which directly affects individual health and quality of lives. Given its potential in posing negative impacts on human welfare, global efforts have been devoted to establishing the rule for trustworthy AI. European Union (EU) set up the Ethics Guidelines~\cite{ec2019ethics} for Trustworthy Artificial Intelligence (AI) as part of its AI strategy. The guideline put forward 7 key requirements, including Non-discrimination, Accountability, Transparency, \textit{etc.}.  Japan also proposes 10 basic principles for implementing and sharing AI in better use. Fairness and accountability are also listed among these principles.

The deep learning models tend to replicate and even amplify this \textit{data bias}, showing discriminant performance against the unprivileged group~\cite{Du2020survey}. For example, existing chest X-ray classifiers are found exhibiting disparities in performance across subgroups distinguished by different phenotypes ~\cite{seyyedkalantari2020chexclusion}. The bias and the consequent disparity exists in all 3 prominent public chest X-ray datasets: MIMIC-CXR~\cite{johnson2019mimic}, Chest-Xray8~\cite{wang2017chestx} and the CheXpert~\cite{irvin2019chexpert}. Similar to the discrimination in face recognition~\cite{wu2019privacy}, dark skin 
patients are under-presented~\cite{Kinyanjui20MICCAI} in existing dermatology datasets: ISIC 2018 Challenge dataset~\cite{tschandl2018ham10000,codella2018skin} and SD-198 dataset~\cite{Sun16ECCVskinbenchmark}. A further study~\cite{Abbasi2020SkinBias} demonstrates that the skin lesion algorithm could show variable performance on subgroups based on age or sex. 

A straightforward solution to alleviate the bias is directly removing the sensitive features.  However, for the medical imaging analysis, these protected attributes are usually not explicitly given to the algorithm. A popular strategy is to utilize adversarial learning to remove discrimination. The first attempt incorporated an adversarial model~\cite{edwards2015censoring} for a discrimination-free representation. Various adversarial objective functions are further proposed~\cite{Zhang2018advlearning} for a different level of group fairness. Recently, a fairness-aware GAN~\cite{xu2018fairgan} is proposed to learn the fair presentation while preserving data utility. 

To the best of our knowledge, yet many methods have been proposed to relieve the discrimination, none of these methods can quantitatively evaluate the bias extent from input data. Since the accountability of trustworthy AI requires to report the potential negative impact, different from the existing works, we propose a novel adversarial learning framework that simultaneously detects and mitigate the bias of arbitrary deep learning-based medical imaging algorithms.

%Disentangling the implicit association between the image and sensitive attributes is an alternative solution~\cite{Du2020survey}.  

\xl{Add orthogonal regulation related work}

==> 6-limitation.tex <==
\section{Discussion}
% ** We are going to first talk about clinical impact and limitations of this work.**
In this paper, we analyze and improve the fairness of deep learning models on a clinical task -- skin lesion classification. Although our adversarial learning strategy show effectiveness of bias mitigation, which reflects on various fairness measurements, we cannot conclude that the model is fair for arbitrary testing cohorts. In compliance with such limitation, we propose a novel fairness prediction (critic module $P$) to estimate the model fairness for a group of inference data. Therefore, model users can evaluate if the deployed model meets their fairness requirement.  As an initial step to study bias mitigation in the medical image analysis, we simplify the bias notations and the sensitive attributes to be binary. In real applications, the categories of sensitive attributes can be more fine-grained. It has great potential to generalize our pipeline to multiple sensitive attributes is the future work.  

==> trash/1-intro-backup.tex <==
\section{Introduction}

%Deep learning algorithms have made impressive achievements and are increasingly deployed in high-risk applications such as medical imaging. A salient question arising is whether we can trust these deep learning models?  If the models are used incorrectly, especially in medical application, the consequence can be irreversible or even fatal. 

The success of deep learning could be partially attributed to its data-driven methodology that automatically learns representation from a large amount of data. However, this end-to-end paradigm leaves the deep learning model vulnerable to the \textit{data bias}: namely, some user groups with \textit{sensitive (protected) attributes} (\textit{i.e.} age or sex) are over or under represented in the deep learning model ~\cite{hardt2016equality,Du2020survey}. As the result, the deep learning models tend to replicate and even amplify this data bias. For example, recent study revealed the discriminant performance on medical imaging-based diagnosis using gender imbalanced in datasets~\cite{larrazabal2020gender}. Existing chest X-ray classifiers are found exhibiting disparities in performance across subgroups distinguished by different phenotype ~\cite{seyyedkalantari2020chexclusion,seyyedkalantari2020chexclusion}. 
%This discrimination has been verified in several medical imaging tasks from chest X-ray~\cite{seyyedkalantari2020chexclusion} to  dermatology~\cite{Kinyanjui20MICCAI}. 
%The bias and the consequent disparity exists in all 3 prominent public chest X-ray datasets: MIMIC-CXR~\cite{johnson2019mimic}, Chest-Xray8~\cite{wang2017chestx} and the CheXpert~\cite{irvin2019chexpert}.  
Similar to the discrimination in face recognition~\cite{wu2019privacy}, dark skin patients may be under-presented~\cite{Kinyanjui20MICCAI} in existing dermatology datasets: ISIC 2018 Challenge dataset~\cite{tschandl2018ham10000,codella2018skin}. A further study~\cite{Abbasi2020SkinBias} demonstrates that the skin lesion algorithm could show variable performance on subgroups. If the decision-making is (partially) based on the sensitive attribute values, the consequence can be irreversible or even fatal, especially in medical application. 


To build trustworthy Artificial Intelligence (AI), global efforts from European Union (EU)~\cite{ec2019ethics}, to the government of Japan~\cite{Japan_ethically_2019} have been instructing that the model should be adherence to ``non-discrimination and fairness". Unfairness mitigation mainly fall in the following three approaches: 1) adversarial learning~\cite{beutel2017data,wang2019balanced,zhang2018mitigating,xu2018fairgan}; 2) calibration~\cite{zhao2017men,hardt2016equality}; 3) incorporating priors into feature attribution~\cite{hendricks2018women,liu2019incorporating}. Adversarial learning approach is considered the most generalizable approach to different bias inducements. 
%then the fair definition can be judged based on whether the decision-making process is treated differently.
%, and  disproportionately harm (benefit) a subgroup of people.
% One of the main causes of  unfairness is referred to \textit{data bias}: some user groups with specific \textit{sensitive (protected) attributes} are over or under represented in the training dataset~\cite{hardt2016equality}. 
%This discrimination has been verified in several medical imaging tasks from chest X-ray~\cite{seyyedkalantari2020chexclusion} to  dermatology~\cite{Kinyanjui20MICCAI}. 
Although there are unfairness mitigation methods proposed in text and natural image analysis, how to mitigate the unfairness in medical imaging has not been well explored. In addition, though there are over 70 fairness metrics~\cite{aif360-oct-2018}, all of them require to know the distribution of labels and protected attributes,  which may not be available for inference data in real healthcare applications.

% \color[red]{The negative impact of these applications may thus be ignored, hindering the accountability~\cite{ec2019ethics,IEEE_ethically_2017,Japan_ethically_2019}.}   

% This hinders the accountability of applications such as real healthcare applications without the protected information. 
%This restriction hinders the accountability~\cite{ec2019ethics,IEEE_ethically_2017,Japan_ethically_2019} of trustworthy AI, as it is hard to assess the negative impacts without knowing all of the required information.
%\xl{Add unfairness mitigation related work}  which may not be available for inference data in real healthcare applications.



%From machine learning~\cite{Zhang2018advlearning} to medical imaging 


%The bias can be caused by skewed sampling, and XXXX (TBC).





%To ensure the trustworthy,



%One essential factor to examine if the model is trustworthy or not is its fairness. 


% 

To enhance the accountability and fairness of artificial intelligence, we propose an adversarial training-based framework. Different from the existing unfairness mitigation work, our proposed pipeline is the first to simultaneously \textbf{mitigate} and  \textbf{detect} the unfairness in the medical image analysis. 
%To mitigate unfairness, the proposed framework transfers the input images into a fair feature domain that is neutral to the sensitive attributes such as age, sex, skin tone, \textit{etc.} Notably, we aim to propose a way to predict (un)fairness without requiring labels and protected attributes information of the inference data.  We achieve the above two goals through a generative adversarial network (GAN) structure-alike domain adversarial alignment training. 
As illustrated in Fig.\ref{fig:structure}, the \textit{discriminator} comprises of two tasks: 1. the \textbf{bias discrimination module} distinguishes between privileged and unprivileged samples, and 2. \textbf{critic prediction module} predicts unfairness of given data. 
%Since the critic module should elaborate on the features relevant to unfairness rather than cracking the discrimination module, we impose an gradient orthogonality regularization~\cite{qi2018global,suteu2019regularizing,du2018adapting} to force two modules to be trained independently on the tangent space in our multi-task learning.
%, thus being independent of each other. Via adversarial alignment training, \textit{feature generator} aims to fool the discrimination module by mapping the feature space of the unprivileged group to the feature space of the privileged group. 
 % Notably, as the generator gradually adjusts the fairness in the transformed space, the critic module can also learn from these samples of various unfairness levels. 
 %The adversarial learning iterations also serve as an argumentation that significantly enhances our model's unfairness prediction ability. 
 Through adversarial training, the \textit{feature generator} can generate discrimination-free features that are served as the inputs for disease \textit{classifier}. 
 %Note that our framework could be used for arbitrary deep learning-based medical imaging classifier.
 We have evaluated our framework on a popular medical imaging task: skin lesion classification. The framework was effective in both predicting and improving the unfairness on the sensitive attributes of age, skin tone, and sex.

Our contributions are summarised into following four folds: 1) This work addresses the neglected fairness problem in medical image analysis and provides unfairness mitigation solutions via adversarial training a discrimination module; 2)  To ensure the accountability of trustworthy AI, we propose to co-train a critic module that is able to estimate unfairness for the inference data without knowing its sensitive attributes; 3) To force the critic module to make fairness estimation independently from bias discrimination, we introduce a novel orthogonality regulation; 4) As an early effort towards fair AI design for medical image analysis, our framework is demonstrated to be effective in predicting and mitigating the unfairness of medical imaging tasks. 
% \xl{Yifan, please help polish this paragraph.}

\begin{comment}
Our contributions are summarised into following four folds:
\begin{itemize}
    \item This work addresses the neglected fairness problem in medical image analysis while providing unfairness mitigation solutions via adversarial training a discrimination module.
    \item To ensure the accountability of trustworthy AI, we propose to co-train a critic module that is able to estimate unfairness for the inference data without knowing its sensitive attributes.
    \item To force the critic module to make fairness estimation independently from bias discrimination, we introduce a novel orthogonality regulation.
    \item As an early effort towards fair AI design for medical image analysis, our framework has shown to be effective in predicting and mitigating the unfairness of medical imaging tasks.
\end{itemize}
\end{comment}

\iffalse
    \item During the training iterations, the detector in the discriminator is able to learn from the samples of a variety of unfairness. In other words, the training data is internally augmented with respect to the unfairness thanks to the adversarial learning structure.
\fi
